Pure Operation-Based Replicated Data Types

Distributed systems designed to serve clients across the world often make use of geo-replication to attain low latency and high availability. Conflict-free Replicated Data Types (CRDTs) allow the design of predictable multi-master replication and support eventual consistency of replicas that are allowed to transiently diverge. CRDTs come in two flavors: state-based, where a state is changed locally and shipped and merged into other replicas; operation-based, where operations are issued locally and reliably causal broadcast to all other replicas. However, the standard definition of op-based CRDTs is very encompassing, allowing even sending the full-state, and thus imposing storage and dissemination overheads as well as blurring the distinction from state-based CRDTs. We introduce pure op-based CRDTs, that can only send operations to other replicas, drawing a clear distinction from state-based ones. Data types with commutative operations can be trivially implemented as pure op-based CRDTs using standard reliable causal delivery; whereas data types having non-commutative operations are implemented using a PO-Log, a partially ordered log of operations, and making use of an extended API, i.e., a Tagged Causal Stable Broadcast (TCSB), that provides extra causality information upon delivery and later informs when delivered messages become causally stable, allowing further PO-Log compaction. The framework is illustrated by a catalog of pure op-based specifications for classic CRDTs, including counters, multi-value registers, add-wins and remove-wins sets.

==> mathdefs.tex <==
\RequirePackage{latexsym}
\RequirePackage{dsfont}



\mathcode`.="613A
\mathcode`|="326A

\let\es=\relax


\newcommand\tx[1]{\hbox{ #1 }}
\newcommand{\defeq}{\stackrel{.}{=}}

\let\vect=\overrightarrow
\let\implies=\Rightarrow
\let\implied=\Leftarrow

\let\sqleq=\sqsubseteq
\let\sqgeq=\sqsupseteq
\let\pleq=\sqleq
\let\pgeq=\sqgeq

\def\land{\mathrel{\wedge}}
\def\lor{\mathrel{\vee}}
\let\bigland=\bigwedge
\let\biglor=\bigvee

\def\preleq{\mathrel{
  \raise 2pt\hbox{$\mathop\sqsubset\limits_{\hbox{$\sim$}}$}%
}}


\let\union=\cup
\let\bigunion=\bigcup
\let\join=\sqcup
\let\bigjoin=\bigsqcup
\let\meet=\sqcap
\newcommand{\down}{\mathord{\downarrow}}
\newcommand{\disjointunion}{\mathbin{\mathaccent\cdot\cup}}

\newcommand\setsize[1]{\left| #1 \right|}
\newcommand\domxtn{\mathbin{\stackrel{+}{|}}}
\newcommand\domainsub{\mathop{\lhd\mkern-14mu-}}


\newcommand{\map}{\mathrel{\hookrightarrow}}
\newcommand\goesto[1]{{\mathop{\longrightarrow}\limits^{#1}}}
\newcommand\goes{\longrightarrow}


\newcommand\auxfun[1]{\expandafter\newcommand\csname #1\endcsname{%
 \mathop{\hbox{$\mathsf{#1}$}}\nolimits}}
 \newcommand\af[1]{\mathop{\hbox{$\mathsf{#1}$}}\nolimits}
 \newcommand\kw[1]{\mathrel{\hbox{$\mathbf{#1}$}}}

\auxfun{Max}
\auxfun{fix}
\auxfun{dom}
\auxfun{fst}
\auxfun{snd}
\auxfun{ran}


\newcommand{\pow}[1]{{\cal P}(#1)}
\newcommand{\bool}{\mathds{B}}
\newcommand{\nat}{\mathds{N}}
\newcommand{\ids}{\mathds{I}}




\newcommand\letin[2]{\mathop{\hbox{$\mathrm{let}$}} #1 \Leftarrow #2 . }
\newcommand\lift[1]{\lfloor #1 \rfloor}

\newcommand\true{\mathrm{true}}
\newcommand\false{\mathrm{false}}


\newcommand\iffdef{\mathrel{\Longleftrightarrow}}
\newcommand\nullstring{\epsilon}
\newcommand\pfunc{\hookrightarrow}
\newcommand\func{\rightarrow}


